Select and Distill: Selective Dual-Teacher Knowledge Transfer for Continual Learning on Vision-Language Models

Large-scale vision-language models (VLMs) have shown a strong zero-shot generalization capability on unseen-domain data. However, adapting pre-trained VLMs to a sequence of downstream tasks often leads to the forgetting of previously learned knowledge and a reduction in zero-shot classification performance. To tackle this problem, we propose a unique Selective Dual-Teacher Knowledge Transfer framework that leverages the most recent fine-tuned and the original pre-trained VLMs as dual teachers to preserve the previously learned knowledge and zero-shot capabilities, respectively. With only access to an unlabeled reference dataset, our proposed framework performs a selective knowledge distillation mechanism by measuring the feature discrepancy from the dual-teacher VLMs. Consequently, our selective dual-teacher knowledge distillation mitigates catastrophic forgetting of previously learned knowledge while preserving the zero-shot capabilities of pre-trained VLMs. Extensive experiments on benchmark datasets demonstrate that our framework is favorable against state-of-the-art continual learning approaches for preventing catastrophic forgetting and zero-shot degradation. Project page: https://chuyu.org/research/snd

==> Algorithms/old_algorithm.tex <==
\begin{algorithm}[tb]
\caption{pFedPG for Efficient and Personalized FL}
\label{alg:algorithm}
\textbf{Input}: Number of communication rounds $T$, $F^*$, $G$, $\textbf{P}_{base}$, $D$, and $N$ sets of $\textbf{P}_n$ and $H_n$, $n \in [1, N]$ \\
\textbf{Data}: $N$ labeled datasets $\mathcal{D}_n$, $n \in [1, N]$\\
\textbf{Output}: $F^*$, $H_n$, $\textbf{P}_n$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $t=0$;
\WHILE{$t$ \textless $T$}
\STATE \textbf{\# Personalized prompt adaptation at clients}
\FOR{$n$ in $1:N$}
\STATE Keep $F^{*}$ freeze;
\STATE Set $\textbf{P}_n=G(\textbf{P}_{base},d_n)$, $d_n \in D$ (Eq.~\eqref{eq:atten});
\STATE Randomly sample a minibatch from $\mathcal{D}_n$;
\STATE Update $H_n$ with $\mathcal{L}_{n}$ (Eq.~\eqref{eq:ce});
\STATE Update $\textbf{P}_n$ by $\mathtt{\widetilde{\textbf{P}}_n}\leftarrow \mathtt{\textbf{P}_n} - \gamma \frac{\partial (\mathcal{L}_{n})}{\partial \mathtt{\textbf{P}_n}}$;
\STATE $\Delta \textbf{P}_n=\widetilde{\textbf{P}_n}-\textbf{P}_n$;
\ENDFOR
\STATE \textbf{\# Personalized prompt generation at the server}
\STATE Receive $\Delta \textbf{P}_n$ from all $N$ clients;
\STATE Update $G$, $\textbf{P}_{base}$, and $D$ by Eq.~\eqref{eq:pg};
\STATE $t = t + 1$;
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> Sections/100_Eval_setup.tex <==
\section{Evaluation Setup}
\label{sec:eval}



% Benefit from training and evaluating over $K$ sequences, we can not only calculate classic sequence-wise metrics, but also a more meaningful task-wise metrics that thoroughly investigate the level of forgetting for each task in different sequences.

% \subsubsection{Sequence-wise Metrics.}
% For a sequence $\calS^k$ contains $K$ tasks, we follow previous standards~\cite{lopez2017gradient, chaudhry2018riemannian, chaudhry2019tiny} to measure the following metrics for CL.

% \issue{Average Accuracy (A)} let $a^k_{i, j} \in [0, 1]$ denote the performance of the model on $j$-th task after the model has been continually trained over $i$ tasks in $\calS^k$. The average accuracy $A^k$ is defined as:
% \begin{equation}
% A^k = \frac{1}{K} \sum_{j=1}^{K} a^k_{K, j}
% \end{equation}

% \issue{Forgetting Measure (F)} Let $f^k_{i, j}$ be the forgetting of the model on $j$-th task after the model has been continually trained over $i$ tasks in $\calS^k$, which is calculated as follows:

% \begin{equation}
%     f_{i, j}^k = \max_{\ell \in \{1, \cdots, i-1\}}a^k_{\ell, j} - a_{i, j}^k
% \end{equation}

% The overall average forgetting measure for $\calS^k$ is then defined as:
% \begin{equation}
%     F^k = \frac{1}{K - 1} \sum_{j=1}^{K-1} f_{K, j}^k
% \end{equation}

% For CL on VLMs, we also aim to measure the overall degradation of zero-shot transferability over unseen tasks. Thus, we define the \emph{Zero-shot Degradation Measure (Z)} as below:

% \issue{Zero-shot Degradation Measure} Let z^k_{i, j} be the 



==> Tables/relatedwork_comparison.tex <==
\begin{table}[t]
    \caption{Comparsion among different methods for Continual Learning}
    \label{tab:comparison}
    \begin{adjustbox}{width=\textwidth,center}
        {
            \setlength{\tabcolsep}{10pt}
            \begin{tabular}{lcccc}
                \bottomrule
                
                \toprule
                {} & Rehearsal-based & Data-free & ZSCL & DTMR (Ours) \\
                \midrule
                Prserve zero-shot & \multirow{2}{*}{\centering\xmark} & \multirow{2}{*}{\centering\xmark} & \multirow{2}{*}{\centering\cmark} & \multirow{2}{*}{\centering\cmark} \\
                transferability & & & & \\
                Avoid catastrophic & \multirow{2}{*}{\centering\cmark} & \multirow{2}{*}{\centering\cmark} & \multirow{2}{*}{\centering\xmark} & \multirow{2}{*}{\centering\cmark} \\
                forgetting & & & & \\
                \bottomrule
    
                \toprule
            \end{tabular}
        }
    \end{adjustbox}
\end{table}
